Leveraging Machine Learning to Alleviate Hubbard Model Sign Problems

Lattice Monte Carlo calculations of interacting systems on non-bipartite lattices exhibit an oscillatory imaginary phase known as the phase or sign problem, even at zero chemical potential. One method to alleviate the sign problem is to analytically continue the integration region of the state variables into the complex plane via holomorphic flow equations. For asymptotically large flow times the state variables approach manifolds of constant imaginary phase known as Lefschetz thimbles. However, flowing such variables and calculating the ensuing Jacobian is a computationally demanding procedure. In this paper we demonstrate that neural networks can be trained to parameterize suitable manifolds for this class of sign problem and drastically reduce the computational cost. We apply our method to the Hubbard model on the triangle and tetrahedron, both of which are non-bipartite. At strong interaction strengths and modest temperatures the tetrahedron suffers from a severe sign problem that cannot be overcome with standard reweighting techniques, while it quickly yields to our method. We benchmark our results with exact calculations and comment on future directions of this work.

==> section/bilinear/order-parameters.tex <==
\subsection{Order Parameters}\label{sec:order parameters}

As mentioned, the antiferromagnetic structure factor \eqref{antiferromagnetic structure factor} is an order parameter for Ne\'{e}l order and the equal-time limit of a two-point function \eqref{Neel correlator} in the sign-alternating constant irrep of bipartite lattices.
Put another way, we can fourier transform in both spatial coordinates and take the highest frequency mode for each (which is the zero momentum doubler).
Such an alternating irrep is always there on a bipartite lattice.

Using our general correlator formulation we get access to many more characterizations of structure (by picking different irreps) at once, and our definition generalizes to non-bipartite lattices immediately (diagonalizing the hopping matrix is what is fundamental about the fourier transform).

We can compute spatially uniform order parameters like mean-squared magnetization
\begin{equation}
    \left\langle m_i^2 \right\rangle = V^{-1} \lim_{\tau\goesto0} C^{ii}_{++}(\tau)
\end{equation}
or ferromagnetic order parameters.

We can construct the charge-density-wave order parameter similarly, substituting the charge density operator for $S^3$, with an intensive order parameter
\begin{equation}
    \text{CDW} = V^{-1} \lim_{\tau\goesto0} C^{\rho\rho}_{--}(\tau)
\end{equation}
Similarly, we can build whole correlators and the order parameters are the zero-time correlators on the diagonal in the irrep basis.

In \Ref{Lang2010} the author defines the antiferromagnetic susceptibility $\chi_{AF}$\footnote{See (1.16), and take careful note of the signs, and of the fact that the sums are over $\ell\neq\ell'$} which we can extract from
\begin{equation}
    \chi_{AF} = V^{-1} \lim_{\tau\goesto0} U_{-x} C^{+-}_{xy}(\tau) U^\dagger_{y-}
\end{equation}
where both spatial indices are projected to the sign-alternating irrep.
We have numerically reproduced \Ref{Lang2010}'s exact result on two spatial sites for a variety of $U$s and $\beta$s.

If the correlations over long distances become very mild and contribute a lot of noise we can again just examine nearest neighbor correlations by tracing the spatial indices with the hopping matrix. (Additional powers of the hopping matrix allow access to longer-range correlations.)

\todo{What about the correlators between $N$ operators in different spatial irreps?}


==> section/bilinear/projection.tex <==
\subsection{Lattice Projection}\label{sec:projection}

On bipartite lattices such as the honeycomb lattice it is common to look at quantities averaged over every lattice site, or quantities averaged over every lattice site with an alternating sign depending on the sublattice.

For example, in \Ref{PhysRevB.78.224416} the authors define the equal-time antiferromagnetic or Ne\'{e}l structure factor
\begin{equation}
    \label{eq:antiferromagnetic structure factor}
    S_{AF} = \frac{1}{V}\sum_{xy} \epsilon_x \epsilon_y \left\langle S^3_x S^3_y \right\rangle
\end{equation}
where $\epsilon_x=\pm1$ depending on the parity of the site (they study a square lattice), and each sum is over space, $V$ is the spatial volume, and $S_{AF}$ is extensive so that $S_{AF}/V$ scales like a constant towards the infinite volume limit.

On lattices that are not bipartite, the lattice sites do not have a definite parity and there is no meaningful sign-alternating averaging, though a straight average remains meaningful.
So, what should we do to discover order?
One sensible strategy that generalizes the sign-alternating averaging is the projection of each spatial index to irreps of the lattice symmetry.

For example, regardless of the lattice geometry, the constant-on-all-sites vector is trivial under the action of the lattice symmetry.\footnote{
There may be other vectors also trivial under the action of the lattice symmetry; the dynamics can mix them.
}
So, a straight average over space amounts to projecting that spatial degree of freedom to this constant vector (up to normalization).
On a bipartite lattice the sign-alternating constant vector is also a one-dimensional representation of the lattice symmetry.

To find vectors of good lattice symmetry we can diagonalize the hopping matrix $h$.  If we can find a unitary matrix $U$ such that $U$ diagonalizes $h$
\begin{equation}
    h_{xy} = (U\adjoint{U}hU\adjoint{U})_{xy} = U_{xi} (E_i \delta_{ij}) \adjoint{U}_{jy}
\end{equation}
then $U$ contains eigenvectors of $h$.
In other words, $U$ transforms us from position space to fourier space, and contains a set of non-interacting modes.
So, the $i$ and $j$ indices runs over lattice modes.

We indicate certain modes with special labels.
For lattices with translational symmetry the constant-everywhere vector is an eigenvector of $h$, and we label it $+$.  For such a lattice that is also bipartite, we label the alternating-sign constant vector $-$, so that
\begin{equation}\label{eq:Neel correlator}
    S_{AF} = \lim_{\tau\goesto0} C^{33}_{--}(\tau),
\end{equation}
as the $1/\sqrt{V}$ vector normalizations conspire to give the required volume factor \eqref{antiferromagnetic structure factor}.

Generically there are $V^2$ numbers required to quantify a two-spatial-index correlator, which can then be diagonalized to yield $V$ eigenvalues and corresponding eigenvectors.
How these eigenvalues depend on spatial information yields spectral information.
Transforming correlation functions with $U$,
\begin{equation}
    C^{uv}_{ij}(\tau) = U_{ax} C^{uv}_{xy}(\tau) \adjoint{U}_{yj}
\end{equation}
can yield great simplification, because if the vectors $i$ and $j$ fall into different irreps their correlation must vanish.
If one can identify which vectors are allowed to mix and which are not, that can greatly simplify the required diagonalization.
For example, in a cubic lattice, two copies of the $E^+$ irrep occur for $\vec{n}^2=5$\cite{Luu:2011ep}, and the dynamics allow these two copies to mix, but they cannot mix with the $A_1^+$ states, or states of any other irrep.
For the triangle, one can read off the required transformation from the three momentum modes \eqref{triangle single particle operators}.

This transformation is good for single-particle (or single-hole) correlation functions and correlation functions between bilinears, for example, but not for multi-particle (or hole) where more than spatial index occurs on each time; in that case one needs the equivalent of Clebsch-Gordan coefficients for the symmetry group of the lattice geometry.

\todo{Meditate on this:}
We can also consider correlations like
\begin{equation}
    C^{uv}_h(\tau)
    =
    \oneover{N_t}\sum_t
    \left\langle S^{u}_{x,t+\tau} h_{xy} S^{v}_{y,t}\right\rangle
\end{equation}
which guarantees that we only count correlations between sites that are nearest neighbors.
This picks up positive

